Deep-learning-driven event reconstruction applied to simulated data from a single Large-Sized Telescope of CTA

When very-high-energy gamma rays interact high in the Earth's atmosphere, they produce cascades of particles that induce flashes of Cherenkov light. Imaging Atmospheric Cherenkov Telescopes (IACTs) detect these flashes and convert them into shower images that can be analyzed to extract the properties of the primary gamma ray. The dominant background for IACTs is comprised of air shower images produced by cosmic hadrons, with typical noise-to-signal ratios of several orders of magnitude. The standard technique adopted to differentiate between images initiated by gamma rays and those initiated by hadrons is based on classical machine learning algorithms, such as Random Forests, that operate on a set of handcrafted parameters extracted from the images. Likewise, the inference of the energy and the arrival direction of the primary gamma ray is performed using those parameters. State-of-the-art deep learning techniques based on convolutional neural networks (CNNs) have the potential to enhance the event reconstruction performance, since they are able to autonomously extract features from raw images, exploiting the pixel-wise information washed out during the parametrization process. Here we present the results obtained by applying deep learning techniques to the reconstruction of Monte Carlo simulated events from a single, next-generation IACT, the Large-Sized Telescope (LST) of the Cherenkov Telescope Array (CTA). We use CNNs to separate the gamma-ray-induced events from hadronic events and to reconstruct the properties of the former, comparing their performance to the standard reconstruction technique. Three independent implementations of CNN-based event reconstruction models have been utilized in this work, producing consistent results.

==> lst_author.tex <==
\scriptsize
\noindent

H. Abe$^{1}$,
A. Aguasca$^{2}$,
I. Agudo$^{3}$,
L. A. Antonelli$^{4}$,
C. Aramo$^{5}$,
T.  Armstrong$^{6}$,
M.  Artero$^{7}$,
K. Asano$^{1}$,
H. Ashkar$^{8}$,
P. Aubert$^{9}$,
A. Baktash$^{10}$,
A. Bamba$^{11}$,
A. Baquero Larriva$^{12}$,
L. Baroncelli$^{13}$,
U. Barres de Almeida$^{14}$,
J. A. Barrio$^{12}$,
I. Batkovic$^{15}$,
J. Becerra González$^{16}$,
M. I. Bernardos$^{15}$,
A. Berti$^{17}$,
N. Biederbeck$^{18}$,
C. Bigongiari$^{4}$,
O. Blanch$^{7}$,
G. Bonnoli$^{3}$,
P. Bordas$^{2}$,
D. Bose$^{19}$,
A. Bulgarelli$^{13}$,
I. Burelli$^{20}$,
M. Buscemi$^{21}$,
M. Cardillo$^{22}$,
S. Caroff$^{9}$,
A. Carosi$^{23}$,
F. Cassol$^{6}$,
M. Cerruti$^{2}$,
Y. Chai$^{17}$,
K. Cheng$^{1}$,
M. Chikawa$^{1}$,
L. Chytka$^{24}$,
J. L. Contreras$^{12}$,
J. Cortina$^{25}$,
H. Costantini$^{6}$,
M. Dalchenko$^{23}$,
A. De Angelis$^{15}$,
M. de Bony de Lavergne$^{9}$,
G. Deleglise$^{9}$,
C. Delgado$^{25}$,
J. Delgado Mengual$^{26}$,
D. della Volpe$^{23}$,
D. Depaoli$^{27,28}$,
F. Di Pierro$^{27}$,
L. Di Venere$^{29}$,
C. Díaz$^{25}$,
R. M. Dominik$^{18}$,
D. Dominis Prester$^{30}$,
A. Donini$^{7}$,
D. Dorner$^{31}$,
M. Doro$^{15}$,
D. Elsässer$^{18}$,
G. Emery$^{23}$,
J. Escudero$^{3}$,
A. Fiasson$^{9}$,
L. Foffano$^{23}$,
M. V. Fonseca$^{12}$,
L. Freixas Coromina$^{25}$,
S. Fukami$^{1}$,
Y. Fukazawa$^{32}$,
E. Garcia$^{9}$,
R. Garcia López$^{16}$,
N. Giglietto$^{33}$,
F. Giordano$^{29}$,
P. Gliwny$^{34}$,
N. Godinovic$^{35}$,
D. Green$^{17}$,
P. Grespan$^{15}$,
S. Gunji$^{36}$,
J. Hackfeld$^{37}$,
D. Hadasch$^{1}$,
A. Hahn$^{17}$,
T.  Hassan$^{25}$,lo
K. Hayashi$^{38}$,
L. Heckmann$^{17}$,
M. Heller$^{23}$,
J. Herrera Llorente$^{16}$,
K. Hirotani$^{1}$,
D. Hoffmann$^{6}$,
D. Horns$^{10}$,
J. Houles$^{6}$,
M. Hrabovsky$^{24}$,
D. Hrupec$^{39}$,
D. Hui$^{1}$,
M. Hütten$^{17}$,
T. Inada$^{1}$,
Y. Inome$^{1}$,
M. Iori$^{40}$,
K. Ishio$^{34}$,
Y. Iwamura$^{1}$,
M. Jacquemont$^{9}$,
I. Jimenez Martinez$^{25}$,
L. Jouvin$^{7}$,
J. Jurysek$^{41}$,
M. Kagaya$^{1}$,
V. Karas$^{42}$,
H. Katagiri$^{43}$,
J. Kataoka$^{44}$,
D. Kerszberg$^{7}$,
Y. Kobayashi$^{1}$,
A. Kong$^{1}$,
H. Kubo$^{45}$,
J. Kushida$^{46}$,
G. Lamanna$^{9}$,
A. Lamastra$^{4}$,
T. Le Flour$^{9}$,
F. Longo$^{47}$,
R. López-Coto$^{15}$,
M. López-Moya$^{12}$,
A. López-Oramas$^{16}$,
P. L. Luque-Escamilla$^{48}$,
P. Majumdar$^{19,1}$,
M. Makariev$^{49}$,
D. Mandat$^{50}$,
M. Manganaro$^{30}$,
K. Mannheim$^{31}$,
M. Mariotti$^{15}$,
P. Marquez$^{7}$,
G. Marsella$^{21,51}$,
J. Martí$^{48}$,
O. Martinez$^{52}$,
G. Martínez$^{25}$,
M. Martínez$^{7}$,
P. Marusevec$^{53}$,
A. Mas$^{12}$,
G. Maurin$^{9}$,
D. Mazin$^{1,17}$,
E. Mestre Guillen$^{54}$,
S. Micanovic$^{30}$,
D. Miceli$^{9}$,
T. Miener$^{12}$,
J. M. Miranda$^{52}$,
L. D. M. Miranda$^{23}$,
R. Mirzoyan$^{17}$,
T. Mizuno$^{55}$,
E. Molina$^{2}$,
T. Montaruli$^{23}$,
I. Monteiro$^{9}$,
A. Moralejo$^{7}$,
D. Morcuende$^{12}$,
E. Moretti$^{7}$,
A.  Morselli$^{56}$,
K. Mrakovcic$^{30}$,
K. Murase$^{1}$,
A. Nagai$^{23}$,
T. Nakamori$^{36}$,
L. Nickel$^{18}$,
D. Nieto$^{12}$,
M. Nievas$^{16}$,
K. Nishijima$^{46}$,
K. Noda$^{1}$,
D. Nosek$^{57}$,
M. Nöthe$^{18}$,
S. Nozaki$^{45}$,
M. Ohishi$^{1}$,
Y. Ohtani$^{1}$,
T. Oka$^{45}$,
N. Okazaki$^{1}$,
A. Okumura$^{58,59}$,
R. Orito$^{60}$,
J. Otero-Santos$^{16}$,
M. Palatiello$^{20}$,
D. Paneque$^{17}$,
R. Paoletti$^{61}$,
J. M. Paredes$^{2}$,
L. Pavletić$^{30}$,
M. Pech$^{50,62}$,
M. Pecimotika$^{30}$,
V. Poireau$^{9}$,
M. Polo$^{25}$,
E. Prandini$^{15}$,
J. Prast$^{9}$,
C. Priyadarshi$^{7}$,
M. Prouza$^{50}$,
R. Rando$^{15}$,
W. Rhode$^{18}$,
M. Ribó$^{2}$,
V. Rizi$^{63}$,
A.  Rugliancich$^{64}$,
J. E. Ruiz$^{3}$,
T. Saito$^{1}$,
S. Sakurai$^{1}$,
D. A. Sanchez$^{9}$,
T. Šarić$^{35}$,
F. G. Saturni$^{4}$,
J. Scherpenberg$^{17}$,
B. Schleicher$^{31}$,
J. L. Schubert$^{18}$,
F. Schussler$^{8}$,
T. Schweizer$^{17}$,
M. Seglar Arroyo$^{9}$,
R. C. Shellard$^{14}$,
J. Sitarek$^{34}$,
V. Sliusar$^{41}$,
A. Spolon$^{15}$,
J. Strišković$^{39}$,
M. Strzys$^{1}$,
Y. Suda$^{32}$,
Y. Sunada$^{65}$,
H. Tajima$^{58}$,
M. Takahashi$^{1}$,
H. Takahashi$^{32}$,
J. Takata$^{1}$,
R. Takeishi$^{1}$,
P. H. T. Tam$^{1}$,
S. J. Tanaka$^{66}$,
D. Tateishi$^{65}$,
L. A. Tejedor$^{12}$,
P. Temnikov$^{49}$,
Y. Terada$^{65}$,
T. Terzic$^{30}$,
M. Teshima$^{17,1}$,
M. Tluczykont$^{10}$,
F. Tokanai$^{36}$,
D. F. Torres$^{54}$,
P. Travnicek$^{50}$,
S. Truzzi$^{61}$,
M. Vacula$^{24}$,
M. Vázquez Acosta$^{16}$,
V.  Verguilov$^{49}$,
G. Verna$^{6}$,
I. Viale$^{15}$,
C. F. Vigorito$^{27,28}$,
V. Vitale$^{56}$,
I. Vovk$^{1}$,
T. Vuillaume$^{9}$,
R. Walter$^{41}$,
M. Will$^{17}$,
T. Yamamoto$^{67}$,
R. Yamazaki$^{66}$,
T. Yoshida$^{43}$,
T. Yoshikoshi$^{1}$,
and
D. Zarić$^{35}$. \\

\noindent
$^{1}$Institute for Cosmic Ray Research, University of Tokyo.
$^{2}$Departament de Física Quàntica i Astrofísica, Institut de Ciències del Cosmos, Universitat de Barcelona, IEEC-UB.
$^{3}$Instituto de Astrofísica de Andalucía-CSIC.
$^{4}$INAF - Osservatorio Astronomico di Roma.
$^{5}$INFN Sezione di Napoli.
$^{6}$Aix Marseille Univ, CNRS/IN2P3, CPPM.
$^{7}$Institut de Fisica d'Altes Energies (IFAE), The Barcelona Institute of Science and Technology.
$^{8}$IRFU, CEA, Université Paris-Saclay.
$^{9}$LAPP, Univ. Grenoble Alpes, Univ. Savoie Mont Blanc, CNRS-IN2P3, Annecy.
$^{10}$Universität Hamburg, Institut für Experimentalphysik.
$^{11}$Graduate School of Science, University of Tokyo.
$^{12}$EMFTEL department and IPARCOS, Universidad Complutense de Madrid.
$^{13}$INAF - Osservatorio di Astrofisica e Scienza dello spazio di Bologna.
$^{14}$Centro Brasileiro de Pesquisas Físicas.
$^{15}$INFN Sezione di Padova and Università degli Studi di Padova.
$^{16}$Instituto de Astrofísica de Canarias and Departamento de Astrofísica, Universidad de La Laguna.
$^{17}$Max-Planck-Institut für Physik.
$^{18}$Department of Physics, TU Dortmund University.
$^{19}$Saha Institute of Nuclear Physics.
$^{20}$INFN Sezione di Trieste and Università degli Studi di Udine.
$^{21}$INFN Sezione di Catania.
$^{22}$INAF - Istituto di Astrofisica e Planetologia Spaziali (IAPS).
$^{23}$University of Geneva - Département de physique nucléaire et corpusculaire.
$^{24}$Palacky University Olomouc, Faculty of Science.
$^{25}$CIEMAT.
$^{26}$Port d'Informació Científica.
$^{27}$INFN Sezione di Torino.
$^{28}$Dipartimento di Fisica - Universitá degli Studi di Torino.
$^{29}$INFN Sezione di Bari and Università di Bari.
$^{30}$University of Rijeka, Department of Physics.
$^{31}$Institute for Theoretical Physics and Astrophysics, Universität Würzburg.
$^{32}$Physics Program, Graduate School of Advanced Science and Engineering, Hiroshima University.
$^{33}$INFN Sezione di Bari and Politecnico di Bari.
$^{34}$Faculty of Physics and Applied Informatics, University of Lodz.
$^{35}$University of Split, FESB.
$^{36}$Department of Physics, Yamagata University.
$^{37}$Institut für Theoretische Physik, Lehrstuhl IV: Plasma-Astroteilchenphysik, Ruhr-Universität Bochum.
$^{38}$Tohoku University, Astronomical Institute.
$^{39}$Josip Juraj Strossmayer University of Osijek, Department of Physics.
$^{40}$INFN Sezione di Roma La Sapienza.
$^{41}$Department of Astronomy, University of Geneva.
$^{42}$Astronomical Institute of the Czech Academy of Sciences.
$^{43}$Faculty of Science, Ibaraki University.
$^{44}$Faculty of Science and Engineering, Waseda University.
$^{45}$Division of Physics and Astronomy, Graduate School of Science, Kyoto University.
$^{46}$Department of Physics, Tokai University.
$^{47}$INFN Sezione di Trieste and Università degli Studi di Trieste.
$^{48}$Escuela Politécnica Superior de Jaén, Universidad de Jaén.
$^{49}$Institute for Nuclear Research and Nuclear Energy, Bulgarian Academy of Sciences.
$^{50}$FZU - Institute of Physics of the Czech Academy of Sciences.
$^{51}$Dipartimento di Fisica e Chimica 'E. Segrè' Università degli Studi di Palermo.
$^{52}$Grupo de Electronica, Universidad Complutense de Madrid.
$^{53}$Department of Applied Physics, University of Zagreb.
$^{54}$Institute of Space Sciences (ICE-CSIC), and Institut d'Estudis Espacials de Catalunya (IEEC), and Institució Catalana de Recerca I Estudis Avançats (ICREA).
$^{55}$Hiroshima Astrophysical Science Center, Hiroshima University.
$^{56}$INFN Sezione di Roma Tor Vergata.
$^{57}$Charles University, Institute of Particle and Nuclear Physics.
$^{58}$Institute for Space-Earth Environmental Research, Nagoya University.
$^{59}$Kobayashi-Maskawa Institute (KMI) for the Origin of Particles and the Universe, Nagoya University.
$^{60}$Graduate School of Technology, Industrial and Social Sciences, Tokushima University.
$^{61}$INFN and Università degli Studi di Siena, Dipartimento di Scienze Fisiche, della Terra e dell'Ambiente (DSFTA).
$^{62}$Palacky University Olomouc, Faculty of Science.
$^{63}$INFN Dipartimento di Scienze Fisiche e Chimiche - Università degli Studi dell'Aquila and Gran Sasso Science Institute.
$^{64}$INFN Sezione di Pisa.
$^{65}$Graduate School of Science and Engineering, Saitama University.
$^{66}$Department of Physical Sciences, Aoyama Gakuin University.
$^{67}$Department of Physics, Konan University.

